High-fidelity 3D Reconstruction of Solar Coronal Physics with the Updated CROBAR Method

We present an extension of the Coronal Reconstruction Onto B-Aligned Regions (CROBAR) method to Linear Force Free Field (LFFF) extrapolations, and apply it to the reconstruction of a set of AIA, MDI, and STEREO EUVI data. The results demonstrate that CROBAR can not only reconstruct coronal emission structures, but also that it can help constrain the coronal field extrapolations via the LFFF's helicity $\alpha$ parameter. They also provide a real-world example of how CROBAR can easily incorporate information from multiple perspectives to improve its reconstructions, and we also use the additional perspectives to help validate the reconstructions. We furthermore touch on the use of real-world emission passbands rather than idealized power-law type ones using DEMs. We conclude with a comparison of CROBAR generated emission to observed emission and those produced with idealized DEM based power-laws. These results further illustrate the promise of CROBAR for real-world applications, and we make available a preliminary release of the software available for download.

==> aastex_journals.tex <==
%AASTEX journal commands
%Copied from version 5.2 (2005) by D. C. Jacobs 2008

\let\jnlatstyle=\rmfamily
\def\refatjnl#1{{\jnlatstyle#1}}%
\newcommand\aj{\refatjnl{AJ}}%
          % Astronomical Journal
\newcommand\actaa{\refatjnl{Acta Astron.}}%
  % Acta Astronomica
\newcommand\araa{\refatjnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\refatjnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\refatjnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\refatjnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\refatjnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\refatjnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\refatjnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\refatjnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\refatjnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\refatjnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\refatjnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\caa{\refatjnl{Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\refatjnl{Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\refatjnl{Icarus}}%
  % Icarus
\newcommand\jcap{\refatjnl{J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\refatjnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\refatjnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\refatjnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\na{\refatjnl{New A}}%
  % New Astronomy
\newcommand\nar{\refatjnl{New A Rev.}}%
  % New Astronomy Review
\newcommand\pra{\refatjnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\refatjnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\refatjnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\refatjnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\refatjnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\refatjnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasa{\refatjnl{PASA}}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\refatjnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\refatjnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\refatjnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{\refatjnl{Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\refatjnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\refatjnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\refatjnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\refatjnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\refatjnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\refatjnl{Nature}}%
          % Nature
\newcommand\iaucirc{\refatjnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\refatjnl{Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\refatjnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\refatjnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\refatjnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\refatjnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\refatjnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\refatjnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\refatjnl{J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\refatjnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\refatjnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\refatjnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\refatjnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\refatjnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\refatjnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\refatjnl{Proc.~SPIE}}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

